QCardEst/QCardCorr: Quantum Cardinality Estimation and Correction

Cardinality estimation is an important part of query optimization in DBMS. We develop a Quantum Cardinality Estimation (QCardEst) approach using Quantum Machine Learning with a Hybrid Quantum-Classical Network. We define a compact encoding for turning SQL queries into a quantum state, which requires only qubits equal to the number of tables in the query. This allows the processing of a complete query with a single variational quantum circuit (VQC) on current hardware. In addition, we compare multiple classical post-processing layers to turn the probability vector output of VQC into a cardinality value. We introduce Quantum Cardinality Correction QCardCorr, which improves classical cardinality estimators by multiplying the output with a factor generated by a VQC to improve the cardinality estimation. With QCardCorr, we have an improvement over the standard PostgreSQL optimizer of 6.37 times for JOB-light and 8.66 times for STATS. For JOB-light we even outperform MSCN by a factor of 3.47.

==> tikzlibrarypgfplots.hvlines.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% title: Draw horizontal and vertical lines that cross an axis
% type: pgfplots library
% author: Antoine Lejay
% date: 2017-08-05
% usage: \usepgfplotslibrary{hvlines}
% licence: LLPL
% version: 0.1
%
% alternatives: see https://tex.stackexchange.com/questions/240642/add-vertical-line-of-equation-x-2-and-shade-a-region-in-graph-by-pgfplots
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % Two keys, `vertical line` and horizontal line` are defined that could be called
% in the options of axis. They took key-values with key `at` for the position and
% `style` for the style of the line.
%
% Example
% \begin{axis}[vertical line={at=2.5,style={blue}},horizontal line={at=1.5,style={dashed,->}}]
%     \addplot table {
% 	    1	1
% 	    2	2
% 	3	3.5};
% \end{axis}
%
\def\pgfplots@last@vertline@pos{0.0} % default value
\tikzset{vertical line/.code={\pgfqkeys{/tikz/vertical line}{#1}}, % execute #1 in the /tikz/vertical line directory
    vertical line style/.style={},
    vertical line={
	at/.store in=\pgfplots@last@vertline@pos, % default value
	style/.style={/tikz/vertical line style/.style={#1}}, % style for the lines
    },
    vertical line/.code={
	\pgfqkeys{/tikz/vertical line}{style={},#1} % read the keys in the /tikz/vertical line directory
	 tikz/execute at begin axis/.append={
	   \draw[vertical line style] let \p1=(axis description cs:0,0), \p2=(axis description cs:0,1), \p3=(axis cs:\pgfplots@last@vertline@pos,0) in (\x3,\y1) -- (\x3,\y2);
       \pgfqkeys{/tikz/vertical line}{style={}}
   },
    },
}

\def\pgfplots@last@horizontalline@pos{0.0} % default value
\tikzset{horizontal line/.code={\pgfqkeys{/tikz/horizontal line}{#1}}, % execute #1 in the /tikz/horizontal line directory
    horizontal line style/.style={},
    horizontal line={
	at/.store in=\pgfplots@last@horizontalline@pos, % default value
	style/.style={/tikz/horizontal line style/.style={#1}}, % style for the lines
    },
    horizontal line/.code={
	\pgfqkeys{/tikz/horizontal line}{style={},#1} % read the keys in the /tikz/horizontal line directory
	 tikz/execute at begin axis/.append={
	   \draw[horizontal line style] let \p1=(axis description cs:0,0), \p2=(axis description cs:1,0), \p3=(axis cs:0,\pgfplots@last@horizontalline@pos) in (\x1,\y3) -- (\x2,\y3);
       \pgfqkeys{/tikz/horizontal line}{style={}}
   },
    },
}
\endinput
% END 

